ViSAGe: A Global-Scale Analysis of Visual Stereotypes in Text-to-Image Generation

Recent studies have shown that Text-to-Image (T2I) model generations can reflect social stereotypes present in the real world. However, existing approaches for evaluating stereotypes have a noticeable lack of coverage of global identity groups and their associated stereotypes. To address this gap, we introduce the ViSAGe (Visual Stereotypes Around the Globe) dataset to enable the evaluation of known nationality-based stereotypes in T2I models, across 135 nationalities. We enrich an existing textual stereotype resource by distinguishing between stereotypical associations that are more likely to have visual depictions, such as `sombrero', from those that are less visually concrete, such as 'attractive'. We demonstrate ViSAGe's utility through a multi-faceted evaluation of T2I generations. First, we show that stereotypical attributes in ViSAGe are thrice as likely to be present in generated images of corresponding identities as compared to other attributes, and that the offensiveness of these depictions is especially higher for identities from Africa, South America, and South East Asia. Second, we assess the stereotypical pull of visual depictions of identity groups, which reveals how the 'default' representations of all identity groups in ViSAGe have a pull towards stereotypical depictions, and that this pull is even more prominent for identity groups from the Global South. CONTENT WARNING: Some examples contain offensive stereotypes.

==> section/rq/visual_attribute_results.tex <==
\subsection{Visual Attribute Analysis} \label{sec:visual_attr_results}

We assessed the visual nature of 1994 attributes present in the SeeGULL dataset. Recognizing the potential limitations associated with majority voting \cite{prabhakaran2021releasing}, we explored different thresholds to determine the degree of visual nature of an attribute. Figure~\ref{fig:visual_attr} presents one such consensus plot for the `visual nature' of attributes.  X-axis demonstrates the consensus labels, and Y-axis indicates the percentage of attributes for which at least 2 out of 3 annotators reached a consensus.

We observe that 20.41\% of the attributes had a `strongly agree' consensus rating from at least 2 annotators, suggesting that these attributes were perceived as extremely visual. Some examples of strongly visual attributes include `blonde haired', `champagne', `dark skin', `elephant', and `fat'. For 22.16\% of the attributes, annotators `agreed' that they were somewhat visual. Attributes like `rich, `poor', `snake charmer', and `swarthy' were included in this category. A roughly equal portion, comprising of 20.26\% of the attributes were considered non-visual where majority of the annotators `disgareed' about their visual nature. Attributes like `professional', `unemployable', `carefree', 'abusive', and `calm' were present in this category. Approximately 7.52\% of the attributes were deemed extremely non-visual as indicated by the 'strongly disagree' label. Some examples include `good sense of humor', `just', and `unintelligent'; and annotators were unsure regarding the visual nature of 0.2\% of the attributes. 

For our subsequent analysis, we exclude all attributes where any annotator expressed uncertainty, disagreement, or strong disagreement regarding the visual nature. Consequently, our `visual attributes' dataset consists solely of attributes for which all annotators either agreed or strongly agreed upon their visual nature, resulting in a selection of 385 out of the original 1994 attributes. We categorize these select attributes as `visual' for our study.


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/visual_attr.png}
    \caption{Consensus of the perceived 'visual nature' of attributes for different values on a Likert Scale ranging from 'Strongly Agree' to 'Strongly Disagree'.}
    \label{fig:visual_attr}
\end{figure}

